Conical SL(3) foams

In the unoriented SL(3) foam theory, singular vertices are generic singularities of two-dimensional complexes. Singular vertices have neighbourhoods homeomorphic to cones over the one-skeleton of the tetrahedron, viewed as a trivalent graph on the two-sphere. In this paper we consider foams with singular vertices with neighbourhoods homeomorphic to cones over more general planar trivalent graphs. These graphs are subject to suitable conditions on their Kempe equivalence Tait coloring classes and include the dodecahedron graph. In this modification of the original homology theory it is straightforward to show that modules associated to the dodecahedron graph are free of rank 60, which is still an open problem for the original unoriented SL(3) foam theory.

==> Images/cf_cube.tex <==
\begin{scope}
  \node (R) at (-2, 2) {$R$};
  \node (Rd) at ( 2, 2) {$R_{\mathcal{D}}$};
  \node (Ra) at (-2, -2) {$R_\alpha$};
  \node (Rad) at ( 2,-2) {$R_{\alpha{\mathcal{D}}}$};
  \node (A) at (0, 4) {$A$};
  \node (Ad) at ( 4, 4) {$A_{\mathcal{D}}$};
  \node (Aa) at (0, 0) {$A_\alpha$};
  \node (Aad) at ( 4,0) {$A_{\alpha{\mathcal{D}}}$};
  \draw[-to] (Ra)  -- (Rad) node [above, midway, font= \small]
  {$\mathcal{D}^{-1}$};
  \draw[->] (A)  -- (Ad) node [midway, above, font= \small]
  {$\mathcal{D}^{-1}$};
  \draw[->] (Aa)  -- (Aad) node [pos=0.7, above, font= \small]
  {$\mathcal{D}^{-1}$};  

  \draw[->] (R) -- (A) node [left, midway, font = \small] {$x$} node
  [right, midway, font = \small] {$:2$};
  \draw[->] (Ra) -- (Aa) node [left, midway, font = \small] {$x$}
  node [right, midway, font = \small] {$:2$};
  \draw[->] (Rd) -- (Ad) node [left, midway, font = \small] {$x$}
  node [right, midway, font = \small] {$:2$};
  \draw[->] (Rad) -- (Aad) node [left, midway, font = \small] {$x$} node
  [right, midway, font = \small] {$:2$};
  
  \draw[->] (R) -- (Ra) node [left, midway, font = \small] {$\alpha$} node
  [right, midway, font = \small] {$:2$};
  \draw[->] (A) -- (Aa) node [left, pos=0.7, font = \small] {$\alpha$} node
  [right, pos=0.7, font = \small] {$:2$};
  \draw[->] (Ad) -- (Aad) node [left, midway, font = \small] {$\alpha$} node
  [right, midway, font = \small] {$:2$};
  
  \draw[white, line width =2mm] (R) -- (Rd);
  \draw[white, line width =2mm] (Rd) -- (Rad);
  
  \draw[->] (R)  -- (Rd) node [pos=0.7, above, font= \small]
  {$\mathcal{D}^{-1}$};

  \draw[->] (Rd) -- (Rad) node [left, pos=0.7, font = \small] {$\alpha$} node
  [right, pos=0.7, font = \small] {$:2$};
  

  
\end{scope}

==> Images/cf_triangle.tex <==
\begin{scope}
    \begin{scope}
        \draw (0,0) -- (90:1);
        \draw (0,0) -- (-30:1);
        \draw (0,0) -- (-150:1);
        \node at (0, -1) {$\Gamma$};
    \end{scope}
    %\node at (2.5, 0) {$\leftrightsquigarrow$}; 
    \begin{scope}[xshift = 5cm]
        \draw (90:0.7) -- (90:1);
        \draw (-30:0.7) -- (-30:1);
        \draw (-150:0.7) -- (-150:1);
        \draw (90: 0.7)--(-30: 0.7) -- (-150: 0.7)-- cycle;
        \node at (0, -1) {$\Gamma'$};
    \end{scope}
\end{scope}

==> algebrasl2.tex <==

%%%%%%%%%%%%%%%%%%%%
% Road map SL(2)
%%%%%%%%%%%%%%%%%%%%

\subsection{Road map for Frobenius extensions in \texorpdfstring{$U(2)$}{U(2)}-equivariant Khovanov homology}
A building block for the Khovanov homology~\cite{MKCatJones, BNCatJones}
is a specific $(1+1)$-dimensional TQFT, corresponding to a commutative
Frobenius algebra of rank two. Different versions of this TQFT exist,
including those studied in  \cite{BNTangle,MKFrobenius} and in many
other papers
\cite{CaprauTangle,vogel2015functoriality,ClarkMorrisonWalkerFunctoriality,BNMorrisonLee}. These different
versions may yield different types of information. The first striking
example is the construction by Rasmussen~\cite{RasmussenSlice} of a lower bound on the
slice genus of knots based on Lee's deformed 2-dimensional TQFT~\cite{Lee}. An attempt to sort through some of these theories, including Bar-Natan's theories~\cite{BNTangle}, has been made in~\cite{MKFrobenius}. In this section, without trying to be all-inclusive, we point out a couple of particularly important variations on the usual $U(2)$-equivariant Frobenius pair $(R,A)$, with $R$ and $A$ being the  equivariant $U(2)$ cohomology groups with $\Z$ coefficients of a point and a 2-sphere, respectively. We will collect the four Frobenius pairs into the diagram below. 

\[
\ttkz[xscale=1.4]{cf_cube}
\]

This is a diagram of four graded Frobenius extensions of degree two  
\begin{equation}\label{eq_4_extensions} 
(R,A), \  (R_{\alpha},A_{\alpha}), \ (R_{\mcD},A_{\mcD}), \ (R_{\alpha\mcD},A_{\alpha\mcD})
\end{equation} 
and maps between them. In each of these extensions $(R_{\ast},A_{\ast})$ Frobenius algebra $A_{\ast}$ is a free graded $R_{\ast}$ module of rank two with a basis $\{1,X\}$, with the trace map $\epsilon:A_{\ast}\lra R_{\ast}$ 
given by 
\begin{equation} \label{eq_trace_map} 
    \epsilon(1)=0, \ \  \epsilon(X)=1.
\end{equation} 

\vspace{0.1in} 

{\bf 1.} The first extension $(R,A)$ consists of graded rings  
\begin{itemize}
    \item $R = \Z[E_1,E_2]$, $\deg(E_1)=2, \deg(E_2)=4.$
    \item $A = R[X]/(X^2-E_1 X + E_2)$, $\deg(X)=2$. 
\end{itemize}
Algebra $A$ is a commutative Frobenius $R$-algebra of rank two with a basis $\{1,X\}$. The trace is given by formula (\ref{eq_trace_map}). 
The comultiplication is 
\begin{eqnarray}\label{equation_comult} 
     \Delta(1) & = & X \otimes 1 + 1\otimes (X-E_1), \\  \Delta(X) & = & X\otimes X - E_2 1\otimes 1.
\end{eqnarray}
Algebra $A$ is a free graded $R$-module with homogeneous basis $\{1,X\}$. 
Elements $X$ and $E_1-X$ in $A$ are roots of the  polynomial  $x^2-E_1 x + E_2$ with coefficients in $R$, and there is an $R$-linear involution of algebra $A$ transposing $X$ and $E_1-X$. Writing the roots as $(r_1,r_2)=(X,E_1-X)$, 
so that 
\begin{equation*}
    r_1+r_2 = E_1, \ \  r_1 r_2 = E_2, 
\end{equation*}
we have 
\begin{eqnarray}\label{equation_comult_roots}
    \Delta(1) & = & r_1 \otimes 1 - 1 \otimes r_2 \ = \ - (r_2
\otimes 1 - 1 \otimes r_1),  \\
\Delta(r_1) & = & r_1 \otimes r_1 - E_2 1\otimes 1, \\
\Delta(r_2) & = & E_2 1\otimes 1 - r_2 \otimes r_2  .
\end{eqnarray}

$R$-algebra $A$ carries an $R$-linear algebra involution $\sigma_0$ which  permutes the roots, $\sigma_0(r_1)=r_2$, 
$\sigma_0(r_2)=r_1$. 
% \begin{eqnarray}\label{equation_comult_roots}
%     \Delta(1) & = & X\otimes 1 + 1\otimes X - E_1 1 \otimes 1  \\
% \Delta(X) & = &-X \otimes X - E_2 1\otimes 1, \\
% \Delta(r_2) & = & \{ r_1 \otimes r_2 - E_2 1\otimes 1,\} 
% \end{eqnarray}

Comultiplication introduces a sign which breaks the symmetry between the two roots, so comultiplication  does not commute with $\sigma_0$. Likewise, the trace map breaks the symmetry between the roots, 
\begin{equation} \label{eq_trace_map_roots} 
    \epsilon(r_1)=1,\ \  \epsilon(r_2)=-1.
\end{equation}
We do have $\epsilon\sigma_0 = - \epsilon$. 

In Figure~\ref{fig:frob} we recall the usual diagrammatic conventions for 2-dimensional TQFTs and commutative Frobenius algebras, with our distinguished  generator $X$ denoted by a dot.
 
\begin{figure}[ht]
  \centering
  \ttkz[scale = 0.35]{cf_frob}
  \caption{Cobordisms and the Frobenius structure maps dictionary.}
  \label{fig:frob}
\end{figure}

The composition of comultiplication and multiplication
\begin{equation}
    m \Delta \ : \ A \lra A\otimes A \lra A , \ 
    m\Delta(1) = m(r_1 \otimes 1 - 1 \otimes r_2)=r_1-r_2
\end{equation}
is an $A$-module map taking  $1$ to the difference  of roots $r_1-r_2$. Consequently, this map is the multiplication by $r_1-r_2$. Thus, a genus one cobordism with one boundary component, when viewed as a cobordism from the empty one-manifold to $\SS^1$, represents the element $r_1-r_2\in A$. 
A two-torus with two boundary components, when viewed as a cobordism between the circles, describes the map $A\lra A$ which is the multiplication by $r_1-r_2$.  

The trace map $\epsilon$ determines an $R$-linear symmetric bilinear form on $A$, 
\[ (,) \ : \ A \otimes A \lra R , \ (a,b) = \epsilon(ab)
\] 
This is a unimodular form on $A$ with  dual bases $(1,X)$ and $(X-E_1,1)$. This pair of dual bases can also be written $(1,r_1)$ and $(-r_2,1)$.  

The identity map on $A$ decomposes in these bases as usual: \begin{equation}\label{eq_id_map}
    a \ = \  r_1\otimes \epsilon(a) - 1 \otimes \epsilon(r_2 a) \ = \  - r_2\otimes \epsilon(a) + 1 \otimes \epsilon(r_1 a), \ a\in A. 
\end{equation}
We can write this identity diagrammatically as the \emph{neck-cutting} relation. 

\[
\cfCircleId{0.4}=
\cfCircleSplit{0.4}{\bullet}{} -
\cfCircleSplit{0.4}{}{\circ}
=
\cfCircleSplit{0.4}{}{\bullet} -
\cfCircleSplit{0.4}{\circ}{},
\qquad \text{with} \qquad
\cfDecSquare{0.3}{\circ} :=
E_1\cfDecSquare{0.3}{} 
-
\cfDecSquare{0.3}{\bullet}. 
\]

Notice that we use a dot of the second type (hollow dot, a little circle with white area inside) to denote the second root $r_2$, borrowing the idea and notation from \cite{beliakova2019functoriality}.

More accurately, a dot ($\bullet$) placed on a vertically positioned annulus denotes the
multiplication by $r_1=X$ operator on $A$, while the dual (or
hollowed) dot ($\circ$) denotes the multiplication by $r_2=E_1-X$. A torus with a boundary component is the difference of a dot and a dual dot on a disk with the same boundary.

\[
\cfGenusOneBdy{0.4} \, = \, \cfCup{0.5}{\bullet} - \cfCup{0.5}{\circ}. 
\]

Note that $r_1-r_2 = 2X - E_1=m\Delta(1)$ is in $A$ but not in $R$. Recall that the discriminant of the quadratic polynomial 
    $x^2-E_1 x + E_2$ is the square of the difference $r_1-r_2$ of roots and belongs to $R$, 
\begin{equation}\label{eq_discriminant} 
        \mcD = (r_1 - r_2)^2 = E_1^2 - 4 E_2  \ \in R. 
\end{equation}
The degree $\deg(\mcD)=4$.

Note that a closed surface of genus two evaluates to $\epsilon(\mcD)=0$, as in~\cite[Section 9.2]{BNTangle}. 
A closed surface of genus three evaluates to  $2\mcD.$

\[
\cfGenusThree{0.4}\ =\ 2 \mcD
\]

Significance of closed genus three surfaces and their evaluation was pointed out in~\cite[Section 9.2]{BNTangle}, where Lee's theory was tied to specializing the value of the closed genus three surface to $8$.  

 Likewise, a surface of genus two with one boundary circle equals a disk times $\mcD$, see below. 
\[
\cfGenusTwoBdy{0.4}\,=\,
\cfGenusTwoCup{0.4}{\bullet}\,=\, \mcD\,\,
\cfCup{0.4}{}.
\]
%Finally, cobordism $T_1^2$, the square of the $T_1$ cobordism, which %is a connected genus two surface with two boundary components, viewed %as a cobordism from a circle to itself, induces the multiplication by %$\mcD$ map on $A$. 

Two-dimensional TQFT $(R,A)$, with its applications to link homology, was introduced by Bar-Natan~\cite{BNTangle}. It's also the theory labelled $(R_5,A_5)$ in~\cite{MKFrobenius}, with parameters $h,t$ there corresponding to $E_1,-E_2$. 
\vspace{0.1in} 

{\bf 2.}
Frobenius  extension $(R_{\mcD},A_{\mcD})$ consists of graded rings   
\begin{itemize}
    \item $R_{\mcD}=R[\mcD^{-1}]=\Z[E_1,E_2,\mcD^{-1}]$, where 
    $\mcD$ is the discriminant, see equation (\ref{eq_discriminant}). Since $\deg(\mcD^{-1})=-4$, graded algebra $R$ is nontrivial in all even degrees. 
    \item $A_{\mcD}=R_{\mcD}[X]/(X^2-E_1 X + E_2)$,
\end{itemize}
Thus, algebra $R_{\mcD}$ is obtained from $R$ by inverting the discriminant element (localizing along it). Algebra $A_{\mcD}= A \otimes_R R_{\mcD}$, so that the Frobenius extension $(R_{\mcD},A_{\mcD})$ is obtained from $(R,A)$ by inverting the discriminant $\mcD$. 
Algebra $A_{\mcD}$ is a free $R_{\mcD}$-module of rank two with a homogeneous basis $\{1,X\}$. 
Formulas (\ref{eq_trace_map}) and (\ref{equation_comult}) for the trace and the comultiplication hold in this Frobenius extension as well as all other formulas derived above for the extension $(R,A)$. 

\vspace{0.07in} 

{\it Separability:} Given a unital homomorphism $\psi: S \lra T$ of commutative rings, one can form the enveloping algebra $T^e=T\otimes_S T$, acting on $T$ by  
\[ (t_1\otimes t_2)t= t_1 t t_2. 
\] 
Homomorphism $\psi$ is called \emph{separable} if there exists a 
homomorphism $\mu:  T\lra T\otimes_S T$ of $T^e$-modules such that 
$m \circ \mu = \mathrm{Id}_T,$
\[ m\circ \mu  \ : \ T  \lra T\otimes_S T \lra T.
\] 

\emph{Remark:} Separability can be defined for noncommutative $S$-algebras $T$ as well, changing the notion of  the enveloping algebra to $T^e=T\otimes_S T^o,$ where $T^o$ is the opposite algebra of $T$. 

Separability is equivalent to the existence of an idempotent $e\in T\otimes_S T$ such that $m(e)=1$ and $e u=0$ for any $u\in\ker(m)$.
Such $e$ is called a \emph{separability idempotent}. Separability is also equivalent to the condition that the exact sequence of $T^e$-modules 
\[ 0 \lra \ker(m) \lra T\otimes_S T \stackrel{m}{\lra} T \lra 0 
\] 
splits. $T^e$-submodule $\ker(m)$ is generated by the complementary idempotent $1-e$. We refer to \cite{Kadison, FordBook} for more information on separable extensions. 

\begin{prop} The ring extension $R_{\mcD}\lra A_{\mcD}$ is separable.
\end{prop} 

\begin{proof} Specializing the above notations to our case, we have the algebra 
\[
A_{\mcD}^e = A_{\mcD} \otimes_{R_{\mcD}} A_{\mcD}.
\] 
Since $m\Delta=(r_1-r_2)\Id_{A_{\mcD}}$, see earlier, and $\mcD=(r_1-r_2)^2$ is invertible in $R_{\mcD}$, we can rescale the comultiplication to the map 
\[ \Delta_{\mcD} \ := \ \ell_{r_1-r_2}\mcD^{-1}\Delta = \ell_{(r_1-r_2)^{-1}}\Delta \ : \ 
A_{\mcD} \lra A_{\mcD}^e 
\]
to split the short exact sequence 
\[ 0 \lra \ker(m) \lra A_{\mcD}\otimes_{R_{\mcD}} A_{\mcD} \stackrel{m}{\lra} A_{\mcD} \lra 0 .
\]
Here $\ell_{r_1-r_2}$ denotes the left multiplication by $r_1-r_2$ on 
$A_{\mcD}^e$, but the right multiplication by the same element works as well, since $\Delta$ is a homomorphism of $A_{\mcD}^e$-modules. Diagrammatically, 
\[
    \Delta_{\mcD}= \mcD^{-1} \cfDelta{0.4}{\star},  \quad \text{with} \quad \cfDecSquare{0.4}{\star} = \cfDecSquare{0.4}{\bullet} - \cfDecSquare{0.4}{\circ}. 
\]

The separability idempotent is 
\begin{align*}
e &= \Delta_{\mcD}(1) =
\mcD^{-1}((r_1-r_2)\otimes 1)(r_1\otimes 1 - 1\otimes r_2) \\
  &=\mcD^{-1}(r_1\otimes 1 - 1 \otimes
  r_2)^2 = \mcD^{-1} \Delta(1)^2. \qedhere
\end{align*}
\end{proof} 

\vspace{0.1in}

{\bf CAN WE DRAW SEPARABILITY IDEMPOTENT HERE AS A GENUS ONE TUBE TIMES $\mcD^{-1}$? SURE. Do you want to skype?Sure.ju
s audio. Sure}

\vspace{0.1in}  

Idempotent $e$ is \emph{strongly separable}, that is, fixed by the involution of $A^e_{\mcD} $ which permutes the two factors in the tensor product \cite[section 5.3]{Kadison}. This is due to $\Delta(1)$ being invariant under this involution. 

\vspace{0.1in} 

{\bf MAY BE MENTION RELATION OF SEPARABILITY AND HOCHSCHILD HOMOLOGY and cite Jozef's paper.} \cite{JPKhoHomHochHom}

\vspace{0.1in} 

{\bf COMPLETE SEPARABILITY STORY} 

\vspace{0.1in} 



{\bf PROBABLY MOVE THIS PARAGRAPH LATER, WHERE WE STUDY SEAMS AND INVOLUTION $\sigma$:}
For comparison, our original extension $R\lra A$ is not separable, since it's easy to check that the multiplication map $m:A\otimes A \lra A$ does not split.  


\vspace{0.1in} 

{\bf 3.}
The third extension $(R_{\alpha},A_{\alpha})$ consists of graded rings   
\begin{itemize}
    \item $R_{\alpha} = \Z[\alpha_1,\alpha_2]$, $\deg(\alpha_1)=\deg(\alpha_2)=2$. 
    \item $A_{\alpha} = R_{\alpha}[X]/((X-\alpha_1)(X-\alpha_2))$, $\deg(X)=2$. 
\end{itemize}
The involution $\alpha_1 \leftrightarrow \alpha_2$ induced by the permutation of indices  acts on $R_{\alpha}$, and we  identify the subring of invariants under this involution  with the ring  $R=\Z[E_1,E_2]$ via identifications $E_1= \alpha_1+\alpha_2, E_2 =\alpha_1\alpha_2$. Under the inclusion $R\subset R_{\alpha}$, the latter is a free graded $R$-module of rank $2$ with a homogeneous basis $\{ 1,\alpha_1\}$, for example. 

Recall that $A$ is a graded $R$-algebra as well. Graded $R$-algebras $A$ and $R_{\alpha}$ are isomorphic, and there are two possible isomorphisms, taking $X\in A$ to either $\alpha_1$ or $\alpha_2$ in $R_{\alpha}$. Notice that $X=r_1,E_1-X=r_2$ in $A$ and $\alpha_1, \alpha_2$ are roots of the polynomial  
$y^2-E_1y+E_2$ with coefficients in $A$, and any $R$-algebra isomorphism $A \cong R_{\alpha}$ will take roots $r_1,r_2$ to roots $\alpha_1,\alpha_2$ in some order. 
Despite the existence of these isomorphisms, rings $A$ and $R_{\alpha}$ have different uses and origins, and we avoid identifying them.

{\bf REWRITE AND MOVE TO WHERE WE DO $A$-bimodules:}
(although such an identification would  allow us to also view $A_{\alpha}$ as the Soergel bimodule associated to the transposition in the symmetric group $S_2$ root system, see equation (\ref{eq_A_alpha}) below).  

We can rewrite the defining relation in $A_{\alpha}$ as 
\[ 0=(X-\alpha_1)(X-\alpha_2) = X^2 - E_1 X + E_2, 
\] 
recognizing the defining relation in $A$, to
 obtain a canonical isomorphism 
\begin{equation}\label{eq_A_alpha} 
 A_{\alpha} \ = \ R_{\alpha}\otimes_R A,
\end{equation}
which can be taken as the definition of $A_{\alpha}$. 

Elements $r_1,r_2\in R$ and $\alpha_1,\alpha_2\in A_{\alpha}$ are roots in $A_{\alpha}$ of $y^2-E_1y+E_2$. Furthermore, we have 
\[ 
r_1+r_2 = \alpha_1 + \alpha_2=E_1, \ r_1r_2 = \alpha_1\alpha_2=E_2.
\] 
The four elements $r_i-\alpha_j$, $i,j\in\{1,2\}$, are zero divisors in $R_{\alpha}$: 
\[ (r_1-\alpha_1)(r_1-\alpha_2) = (X-\alpha_1)(X-\alpha_2) = 0.
\] 
Up to a sign, that's only two zero divisors, since $r_2-\alpha_1= - (r_1 -\alpha_2)$, etc. 

The comultiplication map can be simply written using $X-\alpha_i$, $i=1,2$:  
\begin{eqnarray*}
\Delta(1) & = & (X-\alpha_1) \otimes 1 + 1 \otimes (X-\alpha_2) = (X-\alpha_2) \otimes 1 + 1 \otimes (X-\alpha_1), \\
    \Delta(X-\alpha_1) & = & (X-\alpha_1)\otimes (X-\alpha_1), \\
    \Delta(X-\alpha_2) & = & (X-\alpha_2)\otimes (X-\alpha_2).
\end{eqnarray*}
{\bf MAY BE REMOVE:}
It may be convenient to denote $X_{(1)}=X-\alpha_1, X_{(2)}=X-\alpha_2 \in A_{\alpha}$. On the surface, they can be viewed as shifted dots and are depicted by $\circled{1}$ and $\circled{2}$.  

The comultiplication formulas can be interpreted as simple neck-cutting relations 

\vspace{0.1in} 

{\bf SHALL WE PUT HERE DIAGRAMS OF NECK-CUTTING RULES FOR THIS CASE? Decomposition of a tube, as well as tube decorated by one of $X_{(1)}$, $X_{(2)}$. We can discuss how to denote these shifted dots. Also, shall we draw the relation that two of these shifted dots next to each other are zero?}
\[
\cfCircleId{0.4} =
\cfCircleSplit{0.4}{\circled{1}}{}
+
\cfCircleSplit{0.4}{}{\circled{2}}
=
\cfCircleSplit{0.4}{\circled{2}}{}
+
\cfCircleSplit{0.4}{}{\circled{1}}, \qquad
\cfCircleId[\circled{1}]{0.4}=
\cfCircleSplit{0.4}{\circled{1}}{\circled{1}}, \qquad
\cfCircleId[\circled{2}]{0.4}=
\cfCircleSplit{0.4}{\circled{2}}{\circled{2}}, \qquad
\cfDecSquare{0.4}{\circled{1}\circled{2}} =0.
\]


\vspace{0.1in}

In the ring $R_{\alpha}$ discriminant factorizes, 
$\mcD= (\alpha_1 - \alpha_2)^2.$ Ring $R_{\alpha}$ has an additional symmetry, an involution permuting $\alpha_1$ and $\alpha_2$. 

\vspace{0.1in} 

{\bf WHAT ELSE CAN WE DO WITH THIS EXTENSION? SEE DISCUSSION BELOW.}

We can shift to dot to $X-\alpha_2$ and the dual dot to $\alpha_1-X$, but then their sum is $\alpha_1-\alpha_2$, which is one of the square roots of the determinant, not $E_1$. The  product of these shifted dots is zero. We can check if some relations become nicer using these elements. 

{\bf Move to later?  Note that $\sigma_0$ is defined only later.}
{\emph Involutions $\sigma_0$ and $\sigma_{\alpha}$.} We can extend our symmetry $\sigma_0$ to $A_{\alpha}$, with 
\[ \sigma_0 (X -\alpha_1) = \alpha_2 -X, \ 
\sigma_0(X-\alpha_2) = \alpha_1 - X. 
\] 
Consider the $R$-linear 
involution $\sigma_{\alpha}$ on $R_{\alpha}$ and $A_{\alpha}$ that transposes the roots 
$\alpha_1, \alpha_2$ and fixes $X$:  
\[ \sigma_{\alpha}(\alpha_1)=\alpha_2, \ 
\sigma_{\alpha}(\alpha_2)=\alpha_1, \
\sigma_{\alpha}(X)=X. 
\] 
 Algebra involutions $\sigma_0$ and $\sigma_{\alpha}$ of $A_{\alpha}$ commute, and their composition 
$\sigma_{0\alpha}= \sigma_0\sigma_{\alpha}$ is an involution which has an especially simple behaviour on shifted dots, 
\[ \sigma_{0\alpha} (X -\alpha_1) = \alpha_1 -X, \ 
\sigma_{0\alpha}(X-\alpha_2) = \alpha_2 - X. 
\] 


\emph{Equivariant cohomology:} Passing from $(R,A)$ to $(R_{\alpha},A_{\alpha})$ corresponds to passing from $U(2)$-equivariant cohomology of a point and a 2-sphere to $U(1)\times U(1)$-equivariant cohomology of these topological spaces, where $U(1)\times U(1)$ is a maximal torus in $U(2)$. Group $U(2)$ acts on $\SS^2$ via the identification of the latter with $\mathbb{CP}^1$ and descending from the standard action of $U(2)$ on $\CC^2$.  

\vspace{0.2in} 

{\bf 4.}
The fourth extension $(R_{\alpha\mcD},A_{\alpha\mcD})$ consists of graded rings   
\begin{itemize}
    \item $R_{\alpha\mcD} = \Z[\alpha_1,\alpha_2,(\alpha_1-\alpha_2)^{-1}]$, $\deg(\alpha_1)=\deg(\alpha_2)=2$, 
    \item $A_{\alpha} = R_{\alpha}[X]/((X-\alpha_1)(X-\alpha_2))$, $\deg(X)=2$. 
\end{itemize}
This extension is obtained from the third extension $(R_{\alpha},A_{\alpha})$ by inverting the discriminant $\mcD= (\alpha_1-\alpha_2)^2.$ Equivalently, one can invert $\alpha_1-\alpha_2$. 

Let 
\begin{equation}
    e_1 \ = \frac{X-\alpha_1}{\alpha_2-\alpha_1}, 
    \ \ e_2 \ = \frac{X-\alpha_2}{\alpha_1-\alpha_2}
\end{equation}
These are elements of $A_{\alpha\mcD}$ which are mutually-orthogonal complementary idempotents, 
\begin{equation}
    1= e_1 + e_2, \ e_1^2 = e_1, \ e_2^2=e_2, \ e_1 e_2 = e_2 e_1 = 0. 
\end{equation}
Consequently, the ring $A_{\alpha\mcD}$ decomposes as the direct product 
\begin{equation}
    A_{\alpha\mcD} \ = \ R_{\alpha\mcD}e_1 \times R_{\alpha\mcD}e_2. 
\end{equation}
We have 
\begin{eqnarray}
    & & \Delta(e_1) \ = \ (\alpha_2-\alpha_1)\cdot e_1\otimes e_1   , \ \ \Delta(e_2) \ = \ (\alpha_1-\alpha_2)\cdot e_2\otimes e_2  ,\\
    & & \epsilon(e_1)= (\alpha_2-\alpha_1)^{-1}, \ \ \epsilon(e_2)= (\alpha_1-\alpha_2)^{-1}. 
\end{eqnarray}
{\bf Can we restate E.S.Lee's and Rasmussen's results via this theory?} 

\vspace{0.1in} 

{\bf SHALL WE DRAW THE BIGGER CUBE, WITH MORE INFORMATION IN VERTICES, AROUND HERE? Let's discuss.}

\vspace{0.1in} 

{\bf Summary:}
Let us summarize this diagram of Frobenius extensions. 
Diagonal arrows in the diagram show the four Frobenius extensions (\ref{eq_4_extensions}). 
The four horizonal arrows correspond to localizing each of the four commutative rings $R,A,R_{\alpha},A_{\alpha}$  on the left by inverting the discriminant $\mcD\in R$. Consequently, the two Frobenius extensions on the right side of the diagram are separable. 

Downward vertical arrows denote an extension where we tensor each of the  four rings $R,A,R_{\mcD},A_{\mcD}$ with $R_\alpha$ over $R$. 
In particular, 
\[ A_{\alpha} = A\otimes_R R_{\alpha}, \ 
    R_{\alpha \mcD}= R_{\mcD}\otimes_R R_{\alpha} \ 
    A_{\alpha \mcD} = A_{\mcD}\otimes_R R_{\alpha}.
\] 
Note that $R_{\alpha}$ is a free rank two graded $R$ module with a basis $\{1,\alpha_1\}$ (or $\{1,\alpha_2\}$). In fact, $(R,R_{\alpha})$ is a rank two Frobenius extension isomorphic to the extension $(R,A)$. There are two $R$-algebra isomorphisms $A\cong R_{\alpha}$: one of them takes $X$ to $\alpha_1$ and, necessarily, $E_1-X$ to $\alpha_2$, while the other takes the roots $(X,E_1-X)$ of $x^2-E_1x +E_2$ to $(\alpha_2,\alpha_1)$, correspondingly. 

%%%%%%%%%%%%%%%%%%%%%%%%%%
% Involution sigma_0
%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Involution \texorpdfstring{$\sigma$}{sigma} and Galois action.}
    
Algebra $A$ carries an $R$-linear involution $\sigma_0$ given by $\sigma_0(X)=E_1-X$. As an algebra involution, it satisfies $\sigma_0(1)=1$.  This involution transposes the two roots, 
$\sigma_0(r_1)=r_2, \sigma_0(r_2)=r_1$, and $R$ is the subring of $\sigma_0$-invariants of $A$. Notice that the $(-1)$-eigenspace of $\sigma_0$ is zero, which is not surprising when working over a ground commutative ring $R$ and not over a field. 

Via a base change $R\lra R_{\ast}$ this involution extends to an involution 
$\sigma_0$ of the $R_{\ast}$-algebra $A_{\ast}$, for any of the four Frobenius extensions $(R_{\ast},A_{\ast})$ in (\ref{eq_4_extensions}). In fact, it works for any base change $R\lra R_{\ast}$ of commutative rings, but we restrict to these four cases.  

Involution $\sigma_0$ acts $R_{\ast}$-linearly on the free $R_{\ast}$-module $A_{\ast}$ with a basis $\{1,X\}$. In this basis the action is given by the matrix 
\begin{equation}
    \sigma_0 \ \longmapsto \ \left( \begin{matrix} 1 & E_1 \\ 0 & -1 \end{matrix} \right) 
\end{equation}

Let $A_{\ast}[\sigma_0]$ be the crossed product of $A_{\ast}$ with the group ring of the order two group $\ZZ_2$ generated by $\sigma_0$. Elements of $A_{\ast}[\sigma_0]$ have the form $a_0\cdot 1 + a_1\cdot \sigma_0$, with the multiplication rule that  moving  $\sigma_0$ to the right  of $a\in A_{\ast}$ produces $\sigma_0(a) \cdot \sigma_0$: 
\begin{equation}\label{eq_move_sigma0}
    a \cdot \sigma_0 \cdot b = a\cdot \sigma_0(b)\cdot \sigma_0,  \ a,b\in A_{\ast},\ \ \sigma_0^2=1. 
\end{equation}
This gives an $R_{\ast}$-linear action of the cross product $A_{\ast}[\sigma_0]$ on $A_{\ast}$, that is, a homomorphism 
from the cross-product to the endomorphism algebra
\begin{equation}
    A_{\ast}[\sigma_0] \lra \mathrm{End}_{R_{\ast}}(A_{\ast}) \cong 
    \mathrm{Mat}(2,R_{\ast}), 
\end{equation}
the latter isomorphic to the algebra of $2\times 2$ matrices with coefficients in $R_{\ast}$, where we picked the basis $\{1,X\}$ of $A_{\ast}$ as a free $R_{\ast}$-module. 

Algebra $A_{\ast}[\sigma_0]$ is four-dimensional over $R_{\ast}$, with a basis $\{1, \sigma_0, X, X \sigma_0\}$. Its basis elements act on $A_{\ast}=R_{\ast}\cdot 1 \oplus R_{\ast}\cdot X$ as the following $2\times 2$ matrices.
\begin{equation} \label{eq_4_matrices} 
1 \ \longmapsto \ \left( \begin{matrix} 1 & 0 \\ 0 & 1 \end{matrix} \right) , \ 
    \sigma_0 \ \longmapsto \ \left( \begin{matrix} 1 & E_1 \\ 0 & -1 \end{matrix} \right) , \ 
    X \ \longmapsto \ \left( \begin{matrix} 0 & -E_2 \\ 1 & E_1 \end{matrix} \right) , \ 
    X\sigma_0 \ \longmapsto \ \left( \begin{matrix} 0 & E_2 \\ 1 & 0 \end{matrix} \right) , \
\end{equation}
\begin{dfn}[{\cite[Theorem 12.2.9]{FordBook}}]
Suppose given an extension of commutative rings $S\subset T$ with an involution $\tau$ acting $S$-linearly on $T$ with $S$ the fixed subring and $T$ a projective $S$-module. Then  $(S,T)$ is called a \emph{Galois extension} of commutative rings with the cyclic Galois group $C_2=\{1,\tau\}$ of order two if the natural $S$-algebra homomorphism $T[\tau]\lra \End_S(T)$ is an isomorphism. {\bf [I'LL ADD MORE CITATIONS ABOUT GALOIS EXTENSIONS].} Here $T[\tau]$ is the cross product of $T$ with the group ring of the order two group $\{1,\tau\}$. 
\end{dfn}
  
\begin{prop} $(R_{\ast},A_{\ast})$ is a Galois extension with the cyclic group $\{1,\sigma_0\}$ if and only if the discriminant $\mcD=E_1^2-4E_2$ is invertible in $R_{\ast}$. 
\end{prop} 

\begin{proof} The question is whether the four matrices in  (\ref{eq_4_matrices}) are a basis of the free $R_{\ast}$-module $\mathrm{Mat}(2,R_{\ast})$. Writing down these matrices in the column form, we get the matrix 
%If we decompose the images of $\{1, \sigma_0, X, X \sigma_0\}$ in
%  $\End_{R_{\ast}}(A_\ast)$ along the basis
%  $\left\{\begin{psmallmatrix}
%    1 & 0
%    \\ 0 & 0
%  \end{psmallmatrix},
%    \begin{psmallmatrix}
%    0 & 1
%    \\ 0 & 0
%  \end{psmallmatrix},
%    \begin{psmallmatrix}
%    0 & 0
%    \\ 1 & 0
%  \end{psmallmatrix},
%    \begin{psmallmatrix}
%    0 & 0
%    \\ 0 & 1
%  \end{psmallmatrix} \right\}$.
  \[
   U =  \begin{pmatrix}
      1 & 1 &0 & 0 \\
      0 & E_1 & -E_2 & E_2 \\
      0 & 0 & 1 & 1 \\
      1 & -1 & E_1 & 0
    \end{pmatrix}.
  \]
  A square matrix with coefficients in a  commutative ring $S$ is invertible if and only if its determinant is invertible in $S$. 
The determinant of $U$ is $-\mcD$, thus invertible iff $\mcD$ is. 
\end{proof}

Among our four rings $R_{\ast},$ the discriminant is invertible in $R_{\mcD}$ and $R_{\alpha \mcD}.$

\begin{cor} Extensions $(R_{\mcD},A_{\mcD})$ and $(R_{\alpha\mcD},A_{\alpha\mcD})$ are Galois with the involution $\sigma_0$. Extensions $(R,A)$ and $(R_{\alpha},A_{\alpha})$ are not Galois with this involution. 
\end{cor} 

{\b Field extensions of degree two:} Let $F$ be a field. A homomorphism $\psi:R\lra F$ is determined by $a_1=\psi(E_1),a_2=\psi(E_2)$ in  $F$. To $\psi$ we can associate the base change ring $A_{\psi}= A\otimes_R F,$ which is an $F$-vector space with basis $\{1,X\}$ and multiplication $X^2=a_1 X - a_2$. The pair $(F,A_{\psi})$ is a field extension of degree two iff the 
polynomial $f(y) = y^2-a_1 y + a_2$ is irreducible in $F$, that is, does not have a root. 

Consider the image $\psi(\mcD)=a_1^2-4a_2\in F$ and $A_{\psi}=A\otimes_R F$. Suppose  the canonical 
homomorphism $A\lra A_{\psi}$ extends 
to $A^e = A\otimes_R A \subset 1\otimes A \lra A_{\psi}$ producing a homomorphism 
$A\otimes A \lra A_{\psi},$ denoted $\psi_e$. Since the discriminant $\mcD$ is a square in $A^e$, $\mcD= (r_1-r_2)^2$, in the image $\psi(\mcD) = \psi_e(r_1-r_2)^2$ is a square in $A_{\psi}$. 

Assume that field $F$ has characteristic other than two. Then 
for the $F$-algebra $A_{\psi}$ there are three possibilities
\begin{enumerate}
    \item $A_{\psi}$ is a field. This happens exactly when $\psi(\mcD)=a_1^2-4a_2$ is not a square root in $F$, and then $A_{\psi}\cong  F[\sqrt{\mcD}].$
    \item $A_{\psi}=Fe_1\times Re_2$ is the product of two copies of $F$. This happens when $f(y)$ has two distinct roots $y_1,y_2$ in $F$, with idempotents 
    \begin{equation}
        e_1=\frac{X-y_1}{y_2-y_1}, \ \  \mathrm{and} \ \  
    e_2=\frac{X-y_2}{y_1-y_2}.
    \end{equation} 
    Equivalently, $\psi(\mcD)\not=0 $ has a square root in  $F$. 
    \item $A_{\psi}\cong F[z]/(z^2)$ is a nilpotent extension of $F$ by a nilpotent element of order $2$. Equivalently, 
    $\psi(\mcD)=0$, that is, $a_1^2-4a_2=0$ and  $z= X-\frac{a_1}{2}$. 
\end{enumerate}
Cases (1) and (2) happen when homomorphism $\psi:R\lra F$ extends to localization 
$\psi:R_{\mcD}\lra F$. 
 
Assume that $\mathrm{char}(F)=2$. The image  of the discriminant $\psi(\mcD)=$ For 
for the $F$-algebra $A_{\psi}$ there are the following possibilities
\begin{enumerate}
    \item $A_{\psi}$ is a field. This happens exactly when $\mcD$ is not a square root in $F$. 
    \item $A_{\psi}=Fe_1\times Re_2$ is the product of two copies of $F$. This happens when $f(y)$ has two distinct roots $y_1,y_2$ in $F$, with idempotents 
    \begin{equation}
        e_1=\frac{X-y_1}{y_2-y_1}, \ \  \mathrm{and} \ \  
    e_2=\frac{X-y_2}{y_1-y_2}.
    \end{equation} 
    Equivalently, $\psi(\mcD)\not=0 $ has a square root in  $F$. 
    \item $A_{\psi}\cong F[z]/(z^2)$ is a nilpotent extension of $F$ by a nilpotent element of order $2$. Equivalently, 
    $\psi(\mcD)=0$, that is, $a_1^2-4a_2=0$ and  $z= X-\frac{a_1}{2}$. 
\end{enumerate}{\bf DO WE GET MORE POSSIBILITIES HERE?}
$\psi(\mcD)=a_1^2$ is always a root. 
{\bf Separable vs inseparable extensions here.}
$\psi(\mcD)= a_1^2 - 4 a_2$ is not zero in $F$. 

\vspace{0.1in} 

Equivalent condition, with notations above, ({\bf CHECK AND CITATION}): $S=T^{\sigma_0}$ and there exist $x_1,x_2,y_1,y_2\in T$ such that 
\begin{equation}
     x_1 \sigma(y_1)+ x_2 \sigma(y_2)= \left\{  \begin{array}{ll} 1 & \mathrm{if }\ \sigma=1 \\ 0 & \mathrm{if }\ \sigma=\sigma_0
    \end{array} \right. 
\end{equation}

{\bf DISCUSS HOW THIS CONDITION DIFFERS FROM THE NECK-CUTTING RELATION.}

\vspace{0.2in} 


%%%%%%%%%%%%%%%%%%%%%%%%%%
% Involution sigma
%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Involution \texorpdfstring{$\sigma$}{sigma} and defect lines.}
For a TQFT interpretation, it's convenient to modify $\sigma_0$ to an involution $\sigma$ of $A$ as an $R$-module, not as an algebra, given by 
\[ \sigma(1)=-1, \ \sigma(X) = E_1-X. 
\] 
It transposes the roots $r_1,r_2$, takes $1$ to $-1$, and satisfies 
\begin{equation}
    \epsilon \circ \sigma = - \epsilon, 
\end{equation}
which is dual to the statement $\sigma(1)=-1$. 
Furthermore,  

\begin{equation}
       (\sigma  \otimes \sigma) \circ \Delta \circ \sigma \ =  - \Delta,
\end{equation}
Map $\sigma:A \lra A$ decomposes as {\bf CHECK!}
\begin{equation}\label{eq_sigma_cut}
%    \sigma(a) \ = \  X\epsilon(a) - \epsilon(Xa)
\sigma(a)\ = \ (E_1-X) \epsilon(a) + \epsilon((E_1-X)a) 
\end{equation}
%{\bf Is there a version of this equation for $r_1$? Ideally, we'd want both versions, for $X=r_1$ and for $r_2$. I AGREE. Can we just compute via below: $r_1$ and $r_2$ are not totally symmetric because of value of $\epsilon$}
%{\bf We can consider using $-\sigma$ in place of $\sigma$. To remove sign below. Minus then moves to the other root, $r_2$. May be still better than minus at $r_1$. Let's decide when we skype. Compile and check computation below. Sure. No video, may be? Sure


%I'm not sure to follow. But I trust you. SKype now ?

 %}
which we can rewrite as 
\begin{align*}  (1\otimes\sigma)\Delta(1) &=  (1 \otimes\sigma)(X\otimes 1 +1\otimes (X-E_1)) \\ &= - X \otimes 1 - 1\otimes X = - (X\otimes 1 + 1 \otimes X) \\ &= - (r_1\otimes 1 + 1\otimes r_1) 
\end{align*}
\begin{align*} (\sigma\otimes 1)\Delta(1) & = (\sigma\otimes 1)(X\otimes 1 +1\otimes (X-E_1)) \\ & =(E_1-X)\otimes 1 - 1\otimes (X-E_1) \\ & = (E_1-X)\otimes 1 + 1\otimes (E_1-X) \\& = r_2\otimes 1 + 1\otimes r_2
\end{align*}
We have 
\begin{equation}\label{eq_circ_sigma} 
 m \circ (\sigma\otimes 1) \circ \Delta = 0 = m \circ (1\otimes \sigma) \circ \Delta .
\end{equation}
We can depict involution $\sigma$ is


Denote 
    {\bf DIAGRAMMATIC INTERPRETATION, CHECKERBOARD COLORABILITY.}
This equation leads to a short exact sequence of right $A$-modules {\bf is it really exact?}
\begin{equation}
    0 \lra A(2) \stackrel{\Delta_c}{\lra} A \otimes_R A \stackrel{m}{\lra} A \lra 0
\end{equation}
where ${}_{\sigma}\Delta = (\sigma\otimes 1) \circ \Delta$. 
Both $\Delta$ and $m$ are homomorphisms of $A$-bimodules, but since we put $\sigma$ on the left side, ${}_{\sigma}\Delta$ is a homomorphism of right $A$-modules only. Since $A$ is a free module, this sequence splits, 

{\bf GIVE A MAP BACK} 

{\bf DISCUSS THE STRUCTURE BELOW:}

There is also a sequence of $A$-bimodules 
\begin{equation}\label{eq_intro_A2}
    0 \lra A(2) \stackrel{\Delta_c}{\lra} A \otimes_R A \stackrel{m}{\lra} A \lra 0
\end{equation}
where 
\[ A(2)=A\otimes_R A/(X\otimes 1 - 1\otimes (E_1-X))
\] 
is a quotient of the free rank one $A$-bimodule $A\otimes A$ by the subbimodule generated by $\Delta(1)=r_1\otimes 1 - 1\otimes r_2$. As a left and a right $A$-module $A(2)$ isomorphic to $A$, but left and right actions of $X$ differ {\bf by the involution $\sigma$ CHECK}. Denote by $\underline{1}$ the generator of $A(2)$ which is the image of $1\otimes 1$ under the quotient map. The bimodule map $\Delta_c$ is 
\[ \Delta_c(\underline{1}) = X\otimes 1 - 1 \otimes X =r_1\otimes 1 - 1\otimes r_1 = 1\otimes r_2 - r_2 \otimes 1.
\] 

Diagrammatically, we can interpret $\Delta_c$ as the copants cobordism with a cut by an interval in the middle (\emph{seamed copants}). The cut is part of the defect line for $\sigma$.  The target of this cobordism is a disjoint union of two circles. The source is a circle with two marked points which are the end point of the seam (defect interval). 

\begin{figure}
    \centering
    \ttkz[scale=1]{cf_singular-pants}
    \caption{The seam pants on the left and the seam copants on the right.}
    \label{fig:singular-pants}
\end{figure}

\vspace{0.1in} 

{\bf Insert pictures of seamed pants and seamed copants cobordism.}

{\bf Show picture of circle with 2 marked for $A(2)$. Consider a cup cobordism, a cup with a singular line. Seamed pants cobordisms giving 
associative multiplication $A(2)\otimes_R A(2) \lra A(2)$. Get an associative unital Frobenius algebra structure on $A(2)$. Is it a symmetric algebra isomorphic to $A$?Probably, choose a module isomorphism $A\cong A(2)$. Might get two isomorphisms.}

\vspace{0.1in}

{\bf DISCUSS CIRCLE WITH TWO MARKED POINTS. DRAW. EVALUATION. MORE CANONICAL WAY TO DEFINE $A(2)$ as the state space of a circle with two marked points.}

Use seamed pants surface for a canonical surjection $A\otimes A \lra A(2)$.
Extend this surjection to a short exact sequence dual to (\ref{eq_intro_A2}). 

\vspace{0.1in} 

{\bf MK: I think we can first deal with $\ker(m)$  for $(R,A)$ extension, via seamed copants, and later comment on whether things simplify for $(R_{\mcD},A_{\mcD})$.}
Subspace $\ker(m)\in A\otimes A$ is generated, as $A$-bimodule, by $\kappa = X\otimes 1 - 1 \otimes X$. {\bf It's likely that $\kappa$ equals plus or minus the cup tube with a seamed circle.} 


Furthermore, extension $(R_{\mcD},A_{\mcD})$ has rank two and we can identify $A_{\mcD}$-bimodules $\ker(m)$ and $A_{\mcD}$ to get a short exact sequence of $A_{\mcD}^e$-modules 
\[ 0 \lra A_{\mcD} \stackrel{figure \ out}{\lra} A_{\mcD}\otimes_{R_{\mcD}} A_{\mcD} \stackrel{m}{\lra} A_{\mcD} \lra 0 .
\]
Note that 
\[ \Id_{A_{\mcD}^e} \ = \  \Delta_{\mcD}\circ m +
\Delta_{\mcD}\circ \sigma\circ m
\]
{\bf CHECK; if true, refer to definition of $\sigma$ later. Actually, I think that the term $m\circ (\sigma\otimes Id)\circ \Delta =0$ since it's not checkerboard colorable. In the left arrow above it's tempting to put 
\[ (\sigma\otimes Id)\circ \Delta\ : \  A_{\mcD} \lra A_{\mcD}^e
\]
but it may not be a bimodule map. Think of $\sigma$ as a defect line. 
}
\[ 0 \lra A_{\mcD} \stackrel{figure \ out}{\lra} A_{\mcD}\otimes_{R_{\mcD}} A_{\mcD} \stackrel{m}{\lra} A_{\mcD} \lra 0 .
\] {\bf ADD BACK ARROWS; right back arrow is $\Delta_{\mcD}$}

giving a splitting of this exact sequence. Let us mention a related exact sequence {\bf CHECK!}
\[ 0 \lra A_{\mcD} \stackrel{\Delta}{\lra}
  A_{\mcD}^e
\stackrel{\ell_X-r_X}{\lra} A_{\mcD}^e \stackrel{m}{\lra} A_{\mcD} \lra 0, 
\]
{\bf POSSIBLE CONFUSION BETWEEN ROOTS AND RIGHT MULTIPLICATION}
where $r_X$ denotes the right multiplication by $X$ on $A_{\mcD}^e$ and $\ell_X$ the left multiplication by the same element. {\bf HOW TO SPLIT THIS SEQUENCE.}

\vspace{0.1in} 

{\bf SHOULD WE REWRITE SOME OF THE ABOVE SEQUENCES AS PERIODIC EXACT SEQUENCES, similar to the KM-sequence in the $sl(3)$ case? May be that's for diagrams with boundary.} 

\vspace{0.2in} 

\emph{$GL(2)$ foams and seamed lines:}
 {\bf SHOULD WE DO DIAGRAMMATICS FOR DEFECT LINES CORRESPONDING TO SIGMA? LHR: I THINK IT IS MORE NATURAL TO HAVE LABELEDS 2 FACETS. BUT IN THIS END THIS IS THE SAME. WE WILL CLARIFY THE CONNECTION AT THE END, INCLUDING TWO WAYS TO EVALUATE $GL(2)$ FOAMS.}
 
 

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> algebrasl3.tex <==

%%%%%%%%%%%%%%%%%%%%
%  ROADMAP SL(3) 
%%%%%%%%%%%%%%%%%%%%

%\subsection{Road map for unoriented \texorpdfstring{$SL(3)$}{SL(3)} foam evaluation}
%\label{sec:road_map_3sl}



%%%%%%%%%%%%%%%%%%%
% Subsection on base changes 
%%%%%%%%%%%%%%%%%%%

\section{Base change}
\label{sec:base-change}
\subsection{Universal construction}
Let $R$ be a ring and $\mathcal{C}$ be a cobordism category (we are purposely vague about the definition). There is an empty object denoted $\emptyset_\mathrm{ob}$ and an empty morphism which is the identity of $\emptyset_\mathrm{ob}$ and denoted $\emptyset_\mathrm{mor}$. There is a contravariant involutive functor $\overline{\cdot}\co \mathcal{C} \to \mathcal{C}$ which is the identity on objects which corresponds to changing the orientation (if any) of a cobordism and swaping the roles of the different boundary components.

It is endowed with a monoidal structure coming from disjoint union. A \emph{closed} morphism is an element of $\End_{\mathcal{C}}(\emptyset_{\mathrm{ob}})$.

Suppose given that $\tau\co \End_\mathcal{C}(\emptyset_{\mathrm{ob}}) \to R$. For $\Gamma$ an object of $\mathcal{C}$, define 
$W'(\Gamma)$ to be the free $R$-module generated by $\Hom_{\mathcal{C}}(\emptyset_{\mathrm{ob}})$. Endow $W'(\Gamma)$ with an $R$-bilinear form $( \cdot, \cdot)$ defined elements  of $\Hom_{\mathcal{C}}(\emptyset_{\mathrm{ob}})$ by:
\[
(F_1, F_2) := \tau(\overline{F_2}\circ F_1).
\]

Finally, define $W(\Gamma)= W'(\Gamma)/\ker((\cdot, \cdot))$. This extends for free into a functor $W\co \mathcal{C} \to R\textsf{-Mod}$.

This procedure which constructs $W$ from $\tau$ is known in the litterature is as the \emph{universal construction}. In general this functor is far from being monoidal. Consider for instance the case where $\tau$ is not multiplicative with respect to disjoint union. However in some favorable cases, it produces a TQFT (or TQFT-like) functors see \cite{BHMV, SL3, KR1, RW1}. In the next subsection, we inspect the effect of composing $\tau$ with a ring homomorphism $\psi \co R \to S$.


\subsection{Base change}
\label{sec:base-change-sub}
Suppose given a commutative graded ring $R$ and a free graded $R$-module $W'$ with a homogeneous basis $B'$ with a symmetric $R$-linear grading-preserving bilinear form 
\[ (\cdot,\cdot) \ : \ W' \otimes_R W' \lra R . 
\] 
The form is determined by its values on pairs of basis vectors $(b_1,b_2)$, $b_1,b_2\in B'$.
Denote by  $W = W'/\ker((\cdot,\cdot))$ the quotient of $W'$ by the kernel of the bilinear form. $W$ is a graded $R$-module. 

Let $\psi: R \lra S$ be a unital homomorphism of graded commutative rings. Form the graded free $S$-module
$W'_S = W' \otimes_R S$. As a free $S$-module, it has basis $\{ b\otimes 1\}_{b\in B'}$, and we can write $b$ instead of $b\otimes 1$ when no confusion is possible. Module $W'_S$ comes with a symmetric  $S$-bilinear form with values in $S$ given on basis elements by 
\[ (b_1\otimes 1, b_2\otimes 1) = (b_1,b_2) 
\] 
and extended by $S$-bilinearity. Denote by $W_{\psi}$ of $W_S$ the graded $S$-module which is the quotient of $W'_S$ by the kernel of the bilinear form. There is a natural homomorphism
\begin{equation} \label{eq:quotient_hom} 
   \overline{\psi} \ : \  W \otimes_R S \ \lra \ W_S. 
\end{equation}
This homomorphism is surjective since it is induced by the isomorphism $W'\otimes_R S \stackrel{\cong}{\lra} W'_S.$ In the commutative diagram below, vertical arrows are surjective and the top arrow is an isomorphism. Consequently, the bottom arrow is surjective. 

%{\bf CHANGE ARROWS BELOW TO 'ONTO' ARROWS}

\[
  \tikz[xscale=1.5, yscale=0.8]{
  \node (LT) at (-1, 1) {$W'\otimes_R S$};
  \node (LB) at (-1,-1) {$W\otimes_R S$};
  \node (RT) at ( 1, 1) {$W'_S$};
  \node (RB) at ( 1,-1) {$W_S$};
  \draw (LT) -- (RT) node[midway, above] {$\simeq$};
  \draw[->>] (LT) -- (LB);
  \draw[->>] (RT) -- (RB);
  \draw[->>] (LB) -- (RB) node [midway, below] {$\overline{\psi}$};
  }
\]

% \[
% \begin{CD}
% W'\otimes_R S @>{\cong}>> W'_S  \\
% @V{onto}VV    @VV{onto}V \\
%  W \otimes_R S @>{\overline{\psi},onto}>> W_S
% \end{CD}
% \] 

\vspace{0.1in}

%\emph{Example:} 1.
\begin{exa}
  \begin{enumerate}
    \item
Suppose $R=\kk[x]$, for a field $\kk$, module $W'$ has basis $\{b\}$ and $(b,b)=x$. Then $W=W'=Rb,$ but for the $\kk$-linear homomorphism $\psi:R \lra \kk$, $\psi(x)=0$, the bilinear form on $W_{\kk}$ is identically zero and $W_{\kk}=0$, so that $\overline{\psi}:Rb \otimes_R \kk\cong \kk \lra 0$ has a nontrivial kernel. 
\item Still with $R=\kk[x]$, for the quotient homomorphism $\psi: R\lra \kk[x]/(x^2)$ the module $W=Rb$ is a free $R$-module, but $\kk[x]/(x^2)$-module $W_{\psi}$ is not free. 
\end{enumerate}
\end{exa}
%\vspace{0.1in}

{\bf CHANGE THE NEXT PARAGRAPH. LHR: I'm not quite sure what you meant}

\vspace{0.1in} 

Suppose that $W$ is a \emph{finitely-generated} graded $R$-module. Choose a finite set $Z$ of homogeneous generators of $W$ and  lift it to a finite subset $Z'$ of homogeneous elements of $W'$ via the pull-back of the quotient map $W'\lra W$, so that the restriction of the quotient map to $Z'$ is an isomorphism of sets, $Z'\cong Z$. Each $z'\in Z'$ is a finite linear combination of the elements of $B'$. Let $Y'\subset B'$ be the set of all basis elements that appear with a non-zero coefficient in the expansion of an element of $Z'$ in the basis $B'$. Set $Y'$ is finite. Let $RY'$ be the $R$-submodule of $W'$ generated by $Y'$. It's a free graded $R$-module with a homogeneous basis $Y'$.  Bilinear form $(\cdot,\cdot)$ restricts to a bilinear form on $RY'$ which can be described by a finite matrix with coefficients  in $R$ and rows and columns enumerated by elements of $Y'$.  
\vspace{0.1in} 

$R$-module $W$ comes with an induced bilinear form, which has the trivial kernel on $W$. This bilinear form defines an injective homomorphism of graded $R$-modules 
\[ W \lra W^{\ast}= \Hom_R(W,R). 
\] 

If $W$  is a graded free $R$-module of finite rank, choosing a homogeneous basis of $W$ we can describe the bilinear form via the matrix of its values on pairs of basis vectors. 

We say that $(\cdot,\cdot)$ is \emph{unimodular} on $W$ if $W$ is a free graded $R$-module of finite rank and the homomorphism above is an isomorphism. 

If $W$ is graded free of finite rank, unimodularity is equivalent to the condition that, for a basis as above, the determinant of the Gram matrix of the bilinear form is invertible in $R$. Note that this determinant is always non-zero.

In the Example 1 above, the homomorphism is injective but not surjective. The corresponding matrix is the 1-by-1 matrix $(x)$, and its determinant is not invertible in $R$. 

 

\begin{prop} \label{prop:unimodular}
Suppose that the quotient $W$ is a free graded $R$-module of finite rank and that $(\cdot, \cdot)$ is unimodular
  Then $\overline{\psi}$ is an isomorphism. 
\end{prop}

\begin{proof}
Let $(b_i)_{i\in I}$ be an $R$-basis of $W$. Denote $r\in R^*$ the determinant of the Gram matrix of $(\cdot, \cdot)$ on $(b_i)_{i\in I}$. For $i \in I$, set $b_i^S = \overline{\psi}(b_i) = b_i\otimes S$. 
The determinant of Gram martix on $(b_i^S)_{i\in I}$ of the bilinear form induced by $(\cdot, \cdot)$ on $W_S$ is equal to 
$\psi(r)$. It is invertible hence non-zero. Thus, the family $(b_i^S)_{i\in I}$ is linearly independent and the map $\overline{\psi}$ is injective and therefore induces an isomorphism.
\end{proof}

\begin{prop}\label{prop:SfreeRmodule}
Suppose that the quotient $W$ is a free graded $R$-module of finite rank and that $\psi\co R \to S$ is injective then $\overline{\psi}$ is an isomorphism. 
\end{prop}

\begin{proof}
This goes along the same lines as proof of Proposition~\ref{prop:unimodular}. Here we use the injectivity of $\psi$ to deduce that $\psi(r)$ is not equal to 0.
\end{proof}



Case when $S$ is a free $R$-module under the homomorphism $\psi: R\lra S$. Then $W_S \cong W\otimes_R S.$ 


\vspace{0.2in} 


Recall notations. 

\vspace{0.2in} 

Remind that evaluation is a polynomial. 

\vspace{0.2in} 



